Benchmarking Regression Methods: A comparison with CGAN

In recent years, impressive progress has been made in the design of implicit probabilistic models via Generative Adversarial Networks (GAN) and its extension, the Conditional GAN (CGAN). Excellent solutions have been demonstrated mostly in image processing applications which involve large, continuous output spaces. There is almost no application of these powerful tools to problems having small dimensional output spaces. Regression problems involving the inductive learning of a map, $y=f(x,z)$, $z$ denoting noise, $f:\mathbb{R}^n\times \mathbb{R}^k \rightarrow \mathbb{R}^m$, with $m$ small (e.g., $m=1$ or just a few) is one good case in point. The standard approach to solve regression problems is to probabilistically model the output $y$ as the sum of a mean function $m(x)$ and a noise term $z$; it is also usual to take the noise to be a Gaussian. These are done for convenience sake so that the likelihood of observed data is expressible in closed form. In the real world, on the other hand, stochasticity of the output is usually caused by missing or noisy input variables. Such a real world situation is best represented using an implicit model in which an extra noise vector, $z$ is included with $x$ as input. CGAN is naturally suited to design such implicit models. This paper makes the first step in this direction and compares the existing regression methods with CGAN. We notice however, that the existing methods like mixture density networks (MDN) and XGBoost do quite well compared to CGAN in terms of likelihood and mean absolute error, respectively. Both these methods are comparatively easier to train than CGANs. CGANs need more innovation to have a comparable modeling and ease-of-training with respect to the existing regression solvers. In summary, for modeling uncertainty MDNs are better while XGBoost is better for the cases where accurate prediction is more important.

==> old/OldRelatedWork.tex <==

\subsection{Related work}

Building models that can generate distributions similar to underlying data has been a defining topic of machine learning research. Most generative models assume a parametric distribution over probability density function and maximize likelihood of data. Generative adversarial networks (GAN)~\cite{goodfellow2014generative} and variants~\cite{mirza2014conditional} have demonstrated ability to generate realistic samples of the underlying distribution. GANs use implicit probability modeling without an assumption about probability density function. However, most of this research has been focused on generating realistic images that are characterized by a large structured output space. Little attention has been paid to other class of problems using GANs like regression that typically have a much smaller output space. Regression problems are widely encountered in daily life scenarios, with applications in economics (stock market, housing prices), weather prediction, healthcare (mortality prediction), and mechanics (trajectory estimation). GAN framework has been established as a powerful likelihood free probabilistic generator~\cite{mohamed2016learning,nowozin2016f}.

The closest work to ours is by Zaheer et al.~\cite{zaheergan} for approximating 1D distributions from noise $z$ directly. They however conclude that vanilla GANs and WGANs have a hard time approximating distributions. In this study, we generate continuous output $y$ distribution using $g(x,z)$. Essentially, we use CGAN~\cite{mirza2014conditional} to generate $p(y|x)$ while CGANs have primarily been used for generating images given a class label. Chapfuwa et al.~\cite{chapfuwa2018adversarial} use CGANs with survival analysis for time-to-event modeling. A number of parametric techniques exist for regression. Gaussian Processes~\cite{williams1996gaussian} are one the most extensively used techniques for regression. However, most of models assume a neat additive form of noise. For more complicated noise forms, like hetero-scedastic noise specialized models have be built like hetero-scedastic noise Gaussian Processes~\cite{le2005heteroscedastic}. GANs provide a single framework deploying neural networks as powerful functional approximaters that can handle complex noise forms, as we demonstrate in our experiments. 

While deep neural networks have been extensively used for regression applications, being deterministic models, they suffer from an inability to generate the distributions. GANs can use the deep learning architectures in a probabilistic framework~\cite{mohamed2016learning}. Hence, they can be a powerful tool for regression problems where uncertainty estimation is important. We make such an attempt in this work and show how GANs can be effectively used for regression. 


==> old/problem_statement.tex <==
Multi-output regression~\cite{borchani2015survey} is the problem of predicting multiple related output variables from the given input variables. Multi output regression aims to learn the mapping $f: \mathbf{X} \rightarrow \mathbf{Y}$, where $\mathbf{X}$ is a $n$-dimensional feature space, $\mathbf{X} = (x_1,x_2,\hdots,x_n)$ and $\mathbf{Y}$ is a $m$-dimensional output space, $\mathbf{Y}=(y_1,y_2,\hdots,y_m)$. When $m=1$, the problem reduces to the classical single variable regression problem. We formulate it as a conditional generative problem by using a generator $\hat{Y}=g(X,z)$, where $z \sim (\mu,\sigma) $ is the noise. 

==> old/results-defunct.tex <==
\begin{figure}
\centering
\subfloat[]{\includegraphics[width=.25\textwidth]{images/true_sample_contours_sc7.png}}
\subfloat[]{\includegraphics[width=.25\textwidth]{images/gp_sample_contours_sc7.png}}
\subfloat[]{\includegraphics[width=.25\textwidth]{images/gan_sample_contours_sc7.png}}
\subfloat[]{\includegraphics[width=.25\textwidth]{images/all_mean_ypred_sc7.png}}
\caption{Probability density plots for (a) Generated Data, (b) Gaussian Processes, and (c) CGAN for synthetic data set 1 with Gaussian noise. Mean prediction of these methods with the samples are depicted in (d). Horizontal axis denotes input $x$ and vertical axis denotes output $y$.}% with $y=x+\epsilon$, where $\epsilon \sim \mathrm{exp}(z)$ and $z \sim \mathcal{N}(0,1)$}
\label{fig:sc1}
\end{figure}


\begin{figure}
\centering
\subfloat[]{\includegraphics[width=.25\textwidth]{images/true_sample_contours_sc1.png}}
\subfloat[]{\includegraphics[width=.25\textwidth]{images/gp_sample_contours_sc1.png}}
\subfloat[]{\includegraphics[width=.25\textwidth]{images/gan_sample_contours_sc1.png}}
\subfloat[]{\includegraphics[width=.25\textwidth]{images/all_mean_ypred_sc1.png}}
\caption{Probability density plots for (a) Generated Data, (b) Gaussian Processes, and (c) CGAN for synthetic data set 2. Mean prediction of these methods with the samples are depicted in (d). Horizontal axis denotes input $x$ and vertical axis denotes output $y$.}%with $y = sin(x) + \epsilon$, $\epsilon \sim \mathcal{N}(0,1)$}
\label{fig:sc2}
\end{figure}


\begin{figure}
\centering
\subfloat[]{\includegraphics[width=.25\textwidth]{images/true_sample_contours_sc2.png}}
\subfloat[]{\includegraphics[width=.25\textwidth]{images/gp_sample_contours_sc2.png}}
\subfloat[]{\includegraphics[width=.25\textwidth]{images/gan_sample_contours_sc2.png}}
\subfloat[]{\includegraphics[width=.25\textwidth]{images/all_mean_ypred_sc2.png}}
\caption{Probability density plots for (a) Generated Data, (b) Gaussian Processes, and (c) CGAN for synthetic data set 3 with hetero-scedastic noise. Mean prediction of these methods with the samples are depicted in (d). Horizontal axis denotes input $x$ and vertical axis denotes output $y$.}
\label{fig:sc3}
\end{figure}




\begin{figure}
\centering
\subfloat[]{\includegraphics[width=.25\textwidth]{images/true_sample_contours_sc3.png}}
\subfloat[]{\includegraphics[width=.25\textwidth]{images/gp_sample_contours_sc3.png}}
\subfloat[]{\includegraphics[width=.25\textwidth]{images/gan_sample_contours_sc3.png}}
\subfloat[]{\includegraphics[width=.25\textwidth]{images/all_mean_ypred_sc3.png}}
\newline
\subfloat[]{\includegraphics[width=.25\textwidth]{images/gan_more_sample_ypred_sc3.png}}
\subfloat[]{\includegraphics[width=.25\textwidth]{images/gp_more_sample_ypred_sc3.png}}
\subfloat[]{\includegraphics[width=.25\textwidth]{images/sc3_atx_0-1.png}}
\subfloat[]{\includegraphics[width=.25\textwidth]{images/sc3_atx_0-65.png}}
\caption{Probability density plots for (a) Generated Data, (b) Gaussian Processes, and (c) CGAN for synthetic data set 4 showing Multi Response Regression with hetero-scedastic noise. Mean prediction of these methods with the samples are depicted in (d). Horizontal axis denotes input $x$ and vertical axis denotes output $y$. (e) shows the samples generated from CGAN while (f) shows the samples from Gaussian Processes. (g) and (h) show the probability density plots of $y$ at $x=0.1$ and $x=0.65$ respectively. }
\label{fig:sc4}
\end{figure}



\begin{figure}
\centering
\subfloat[]{\includegraphics[width=.25\textwidth]{images/sinus_ablation.png}}
\subfloat[]{\includegraphics[width=.25\textwidth]{images/sinus_1.png}}
\subfloat[]{\includegraphics[width=.25\textwidth]{images/sinus_5.png}}
\newline
\subfloat[]{\includegraphics[width=.25\textwidth]{images/multi_ablation.png}}
\subfloat[]{\includegraphics[width=.25\textwidth]{images/multi_1.png}}
\subfloat[]{\includegraphics[width=.25\textwidth]{images/multi_8.png}}
\caption{Ablation study on input noise dimension: (a) and (d) show variation of NLPD with the dimension of the input noise respectively for dataset 2 and 4; (b) and (e) show the output prediction of GAN for $\text{dim}(z)=1$; (c) and (f) show the output prediction of GAN for the best dimension found in $[1, 10]$}
\label{fig:sc5}
\end{figure}

\begin{figure}
\centering
\subfloat[]{\includegraphics[width=.25\textwidth]{images/sinus_ablation_trng.png}}
\subfloat[]{\includegraphics[width=.25\textwidth]{images/multi_ablation_trng.png}}
\caption{Ablation study on size of training data for a) dataset 2 b) dataset 4. Reported NNLH is taken to be the mean over 10 runs. We notice that GAN is very robust to the number of training points in the dataset.}
\label{fig:sc6}
\end{figure}


==> sections/notes.tex <==
\paragraph{Introduction:} Start with motivating example in finance, weather, health-care. The real world processes are stochastic and can exhibit non-linear noisy behaviours. The idea is to create a single model that can model all scenarios of multivariate input and multi-output by learning over manifolds the data lies on, taking care of the structure of noise which can be non-linear in the real world. For state-of-the-art methods like Gaussian Processes, we have to build models that cater to different scenarios.  The current models assume a neat additive form of noise: $y=f(x)+\epsilon$. However, in real world the noise can be much more complicated - it can be multi-modal. GANs are capable of handling such noise form.

\paragraph{Pitch for implicit models} Most of real world phenomenon are stochastic in nature. These are the problems that have real world applications and we want to concentrate on these problems. This brings an element of events that can be uncertain (``noisy") in nature and are important to be modeled correctly. Given the above premise of simple additive noise form assumption, these methods are not adequate for modeling such complex phenomenon with complex noise structures. Hence, we want to model the likelihoods correctly. This naturally brings us to KL divergence. However, any this requires estimating true distribution $p(y|x)$ with $q(y|x)$ for KL divergence computation. Non-parametric models can't do this estimation directly since we need to have a closed form expression for $p(y|x)$, while in the real world we only have finite amount of samples without any knowledge about the underlying generator distribution, $p(y|x)$. 

\paragraph{Generative Adversarial Networks} In the original GAN paper Goodfellow et al~\cite{goodfellow2014generative} had shown that a min-max game between the generator and discriminator with a cross entropy loss is similar to minimizing Jennsen Shannon divergence. Nowozin et al.~\cite{nowozin2016f} and Mohamed et al.~\cite{mohamed2016learning} show that family of generator functions can act as proxy for minimizing likelihood functions. We need to justify the relation with minimizing KL divergence here.

\begin{itemize}
    \item Not the goal: Right Practical design in terms of optimization algorithm. 
    \item Main goal: Producing quality error bars by using generative modeling
    \item Amount of data is not an issue, we assume plenty of data
\end{itemize}

